Randomized Asymmetric Chain of LoRA: The First Meaningful Theoretical Framework for Low-Rank Adaptation

Fine-tuning has become a popular approach to adapting large foundational models to specific tasks. As the size of models and datasets grows, parameter-efficient fine-tuning techniques are increasingly important. One of the most widely used methods is Low-Rank Adaptation (LoRA), with adaptation update expressed as the product of two low-rank matrices. While LoRA was shown to possess strong performance in fine-tuning, it often under-performs when compared to full-parameter fine-tuning (FPFT). Although many variants of LoRA have been extensively studied empirically, their theoretical optimization analysis is heavily under-explored. The starting point of our work is a demonstration that LoRA and its two extensions, Asymmetric LoRA and Chain of LoRA, indeed encounter convergence issues. To address these issues, we propose Randomized Asymmetric Chain of LoRA (RAC-LoRA) -- a general optimization framework that rigorously analyzes the convergence rates of LoRA-based methods. Our approach inherits the empirical benefits of LoRA-style heuristics, but introduces several small but important algorithmic modifications which turn it into a provably convergent method. Our framework serves as a bridge between FPFT and low-rank adaptation. We provide provable guarantees of convergence to the same solution as FPFT, along with the rate of convergence. Additionally, we present a convergence analysis for smooth, non-convex loss functions, covering gradient descent, stochastic gradient descent, and federated learning settings. Our theoretical findings are supported by experimental results.

==> name.tex <==
import numpy as np
from sklearn import datasets
import matplotlib.pyplot as plt
from tqdm import tqdm
import torch
import copy
from scipy.linalg import qr
from sklearn.random_projection import GaussianRandomProjection


# A,b = datasets.load_svmlight_file("abalone.txt")
A, b = datasets.make_regression(n_samples=4000, n_features=100, n_informative=100, bias=2.0, tail_strength=0.5, effective_rank=10 )
# , tail_strength=0.5
# print(A.shape)

# A = np.array(A.todense())
print(A.shape)
A_pretrained = np.array(A[0:3000])
b_pretrained = np.array(b[0:3000])

A_finetuned = np.array(A[3000:4000])
b_finetuned = np.array(b[3000:4000])

# A = np.array(A[0:4000])
# b = np.array(b[0:4000])
n_pret = A_pretrained.shape[0]
d_pret = A_pretrained.shape[1]

print(n_pret, d_pret)

n_ft = A_finetuned.shape[0]
d_ft = A_finetuned.shape[1]
# print(n,d)

# Setting the l2 regularizer 
 
lambda_2_pret = 0.0001 * np.max(np.linalg.eigvalsh(A_pretrained.T @ A_pretrained / n_pret))

# Calculating strong convexity and L-smoothness constants 

mu_pret = np.min(np.linalg.eigvalsh(A_pretrained.T @ A_pretrained / n_pret)) + lambda_2_pret

L_pret = np.max(np.linalg.eigvalsh(A_pretrained.T @ A_pretrained / n_pret)) + lambda_2_pret
print('mu_pret, L_pret')
print(mu_pret, L_pret)

# Calculating individual L_i - smoothness constants 

L_i_pret = np.diag(A_pretrained @ A_pretrained.T) + lambda_2_pret

# print(L_i[0])

# Calculating the optimal point (solution)

x_star_pret = np.linalg.inv(A_pretrained.T @ A_pretrained + n_pret * lambda_2_pret * np.eye(d_pret)) @ A_pretrained.T @ b_pretrained


def grad(x, idx):
    return A_pretrained[idx].T @ (A_pretrained[idx] @ x - b_pretrained[idx]) / len(idx) + lambda_2_pret * x

def func_value(x):
    return (1/(2*len(A_pretrained)))*(np.linalg.norm(A_pretrained@x-b_pretrained))**2+(lambda_2_pret/2)*np.linalg.norm(x)**2

def grad_full(x):
    return A_pretrained.T @ (A_pretrained @ x - b_pretrained) / n_pret + lambda_2_pret * x
def grad_us(x):
    idx = np.random.choice(list(range(n_pret)), size = 1, replace=True)
    return grad(x, idx)

def grad_is(x):
    idx = np.random.choice(list(range(n_pret)), size = 1, replace=True, p=L_i_pret / np.sum(L_i_pret))
    return grad(x, idx)

# Implementing full_batch centralized GD method

def gd(x_0, gamma, max_iter = 10000):
    x_k = np.copy(x_0)
    list_of_norms = [np.linalg.norm(x_k - x_star_pret) ** 2]
    list_of_points = [x_0]
    list_of_losses = [func_value(x_0) - func_value(x_star_pret)]
    for k in tqdm(range(int(max_iter))):
        x_k -= gamma * grad_full(x_k)
        list_of_norms.append(np.linalg.norm(x_k - x_star_pret) ** 2 )
        list_of_points.append(x_k)
        list_of_losses.append(func_value(x_k) - func_value(x_star_pret))

    return list_of_points, list_of_norms, list_of_losses

# list_of_points, list_of_norms, list_of_losses = gd(np.ones(d_pret), 1/L_pret, 300000)

# plt.plot(list_of_norms)
# plt.yscale('log')
# plt.savefig('test-test.pdf')









# ========================================================================

lambda_2_ft = 0.001*np.max(np.linalg.eigvalsh(A_finetuned.T @ A_finetuned / n_ft)) 

# Calculating strong convexity and L-smoothness constants 

mu_ft = np.min(np.linalg.eigvalsh(A_finetuned.T @ A_finetuned / n_ft)) + lambda_2_ft

L_ft = np.max(np.linalg.eigvalsh(A_finetuned.T @ A_finetuned / n_ft)) + lambda_2_ft
print('mu_ft, L_ft')
print(mu_ft, L_ft)

# Calculating individual L_i - smoothness constants 

L_i_ft = np.diag(A_finetuned @ A_finetuned.T) + lambda_2_ft

# print(L_i[0])

# Calculating the optimal point (solution)

x_star_ft = np.linalg.inv(A_finetuned.T @ A_finetuned + n_ft * lambda_2_ft * np.eye(d_ft)) @ A_finetuned.T @ b_finetuned

# print(np.reshape(x_star_ft, (2,4)))
# print(x_star_pret)

def grad_ft(x, idx):
    return A_finetuned[idx].T @ (A_finetuned[idx] @ x - b_finetuned[idx]) / len(idx) + lambda_2_ft * x

def func_value_ft(x):
    return (1/(2*len(A_finetuned)))*(np.linalg.norm(A_finetuned@x-b_finetuned))**2+(lambda_2_ft/2)*np.linalg.norm(x)**2

def grad_full_ft(x):
    return A_finetuned.T @ (A_finetuned @ x - b_finetuned) / n_ft + lambda_2_ft * x
def grad_us_ft(x):
    idx = np.random.choice(list(range(n_ft)), size = 1, replace=True)
    return grad_ft(x, idx)

def grad_is_ft(x):
    idx = np.random.choice(list(range(n_ft)), size = 1, replace=True, p=L_i_ft / np.sum(L_i_ft))
    return grad_ft(x, idx)

# ======================================================================================================

def ProxLora(W_0, alpha, inner_step_size, iter_max_sub, max_iter, gamma, rank, d_ft, d_mat_ft, mean, std, track=False):
    current_matrix = W_0
    d_mat_ft = current_matrix.shape[0]
    list_of_points_w = []
    
    for t in tqdm(range(max_iter)):
        W_k = copy.deepcopy(current_matrix)
        
        # print(k)
        
        S_k = np.random.normal(mean, std, size=(d_mat_ft, rank))
        current_Z = solve_subproblem(W_k, current_matrix, S_k, iter_max_sub, inner_step_size, gamma, rank, d_ft, d_mat_ft)
        W_k += S_k@current_Z
        current_matrix = current_matrix + alpha*(W_k - current_matrix)
        if track:
            for j in range(iter_max_sub):
                list_of_points_w.append(np.reshape(current_matrix, (d_ft,)))
        else:
            list_of_points_w.append(np.reshape(current_matrix, (d_ft,)))
        
        # list_of_points_w.append(np.reshape(current_matrix, (8,)))
        

    

    return list_of_points_w



def solve_subproblem(W_cur, W, S, iter_max_sub, step_size, gamma, rank, d_ft, d_mat_ft):
    Z_0 = np.zeros((rank, d_mat_ft))
    
    Z_cur = Z_0
    for j in range(iter_max_sub):
        delta = np.reshape(W_cur + S@Z_cur, (d_ft,))
        Z_cur = Z_cur - step_size* S.T @ (np.reshape(grad_full_ft(delta), (d_mat_ft, d_mat_ft)) + (1./gamma)*(W_cur+S@Z_cur - W))
    return Z_cur


    
  



def RandChain_Lora_Lin(W_0, alpha, step_size, max_iter, rank, d, d_mat, mean, std):
    current_matrix = W_0
    d_mat = current_matrix.shape[0]
    list_of_points_w = []
    list_of_values_w = []
    
    for t in tqdm(range(max_iter)):
        W_k = copy.deepcopy(current_matrix)
        S_k = np.random.normal(mean, std, size=(d_mat, rank))
        delta = np.reshape(W_k, (d,))
        W_k += -step_size * S_k @ np.linalg.inv(S_k.T @ S_k) @ S_k.T @ np.reshape(grad_full_ft(delta), (d_mat, d_mat))
        # for k in range(0, k_max):
        #     # print(k)
        #     list_of_points_w.append(np.reshape(current_matrix, (d,)))
        #     list_of_values_w.append(log_loss(np.reshape(current_matrix, (d,))))
        #     S_k = np.random.normal(mean, std, size=(d_mat, rank))
        #     current_Z = solve_subproblem(W_k, current_matrix, S_k, iter_max_sub, inner_step_size, gamma, rank, d, d_mat)
        #     W_k += S_k@current_Z
        current_matrix = current_matrix + alpha*(W_k - current_matrix)
        list_of_points_w.append(np.reshape(current_matrix, (d,)))
        list_of_values_w.append(func_value_ft(np.reshape(current_matrix, (d,))))
        # list_of_points_w.append(np.reshape(current_matrix, (8,)))
        

    

    return list_of_points_w, list_of_values_w


def RandChain_Lora_Lin_Orth(W_0, alpha, step_size, max_iter, rank, d, d_mat):
    current_matrix = W_0
    d_mat = current_matrix.shape[0]
    list_of_points_w = []
    list_of_values_w = []
    
    for t in tqdm(range(max_iter)):
        W_k = copy.deepcopy(current_matrix)
        Mat = np.random.rand(d_mat, d_mat)
        U, _, _ = np.linalg.svd(Mat)
        S_k = U[:, : rank]

        # S_k = np.random.normal(mean, std, size=(d_mat, rank))
        delta = np.reshape(W_k, (d,))
        W_k += -step_size * S_k @ np.linalg.inv(S_k.T @ S_k) @ S_k.T  @ np.reshape(grad_full_ft(delta), (d_mat, d_mat))
        # for k in range(0, k_max):
        #     # print(k)
        #     list_of_points_w.append(np.reshape(current_matrix, (d,)))
        #     list_of_values_w.append(log_loss(np.reshape(current_matrix, (d,))))
        #     S_k = np.random.normal(mean, std, size=(d_mat, rank))
        #     current_Z = solve_subproblem(W_k, current_matrix, S_k, iter_max_sub, inner_step_size, gamma, rank, d, d_mat)
        #     W_k += S_k@current_Z
        current_matrix = current_matrix + alpha*(W_k - current_matrix)
        list_of_points_w.append(np.reshape(current_matrix, (d,)))
        list_of_values_w.append(func_value_ft(np.reshape(current_matrix, (d,))))
        # list_of_points_w.append(np.reshape(current_matrix, (8,)))
        

    

    return list_of_points_w, list_of_values_w

def RandChain_Lora_Lin_Unifrom(W_0, alpha, step_size, max_iter, rank, d, d_mat):
    current_matrix = W_0
    d_mat = current_matrix.shape[0]
    list_of_points_w = []
    list_of_values_w = []
    
    for t in tqdm(range(max_iter)):
        W_k = copy.deepcopy(current_matrix)
        S_k = np.random.rand(d_mat, rank)
        # Mat = np.random.rand(d_mat, d_mat)
        # U, _, _ = np.linalg.svd(Mat)
        # S_k = U[:, : rank]
        H_t =  S_k @ np.linalg.inv(S_k.T @ S_k) @ S_k.T 
        # S_k = np.random.normal(mean, std, size=(d_mat, rank))
        delta = np.reshape(W_k, (d,))
        W_k += -step_size * H_t@(np.reshape(grad_full_ft(delta), (d_mat, d_mat)))
        # for k in range(0, k_max):
        #     # print(k)
        #     list_of_points_w.append(np.reshape(current_matrix, (d,)))
        #     list_of_values_w.append(log_loss(np.reshape(current_matrix, (d,))))
        #     S_k = np.random.normal(mean, std, size=(d_mat, rank))
        #     current_Z = solve_subproblem(W_k, current_matrix, S_k, iter_max_sub, inner_step_size, gamma, rank, d, d_mat)
        #     W_k += S_k@current_Z
        current_matrix = current_matrix + alpha*(W_k - current_matrix)
        list_of_points_w.append(np.reshape(current_matrix, (d,)))
        list_of_values_w.append(func_value_ft(np.reshape(current_matrix, (d,))))
        # list_of_points_w.append(np.reshape(current_matrix, (8,)))
        

    

    return list_of_points_w, list_of_values_w
# gamma = 1/n_ft

# list_of_z, Z_last = solve_subproblem(np.reshape(x_star_pret, (2,4)),
#                                     np.reshape(x_star_pret, (2,4)),
#                                     np.random.normal(1, 2.5, size=(2, 1)),
#                                     10000,
#                                     1/(1000*(L_ft+1./gamma)),
#                                     gamma)
# list_of_norms_z = []
# for z in list_of_z:
#     list_of_norms_z.append(func_value_ft(np.reshape(np.random.normal(1, 2.5, size=(2, 1))@z, (8,))))

# plt.plot(list_of_norms_z)
# plt.yscale('log')
# plt.savefig('test_z.pdf')


d_mat_ft = 10

W_0_pret = np.reshape(x_star_pret, (d_mat_ft, d_mat_ft))


gamma = 10000*n_ft


list_of_points_w_0 = ProxLora(W_0=W_0_pret, 
                            alpha=1,
                            inner_step_size=0.05/(L_ft+(1./gamma)),
                            iter_max_sub=1,
                            max_iter=3000,
                            gamma = gamma,
                            rank=1,
                            d_ft=d_ft,
                            d_mat_ft=d_mat_ft,
                            mean = 1,
                            std = 2.5,
                            track = True)

list_of_values_w_0 = []
for point in list_of_points_w_0:
    list_of_values_w_0.append(func_value_ft(point) - func_value_ft(x_star_ft))


gamma = 10000*n_ft


list_of_points_w_1 = ProxLora(W_0=W_0_pret, 
                            alpha=1,
                            inner_step_size=0.035/(L_ft+(1./gamma)),
                            iter_max_sub=3,
                            max_iter=1000,
                            gamma = gamma,
                            rank=1,
                            d_ft=d_ft,
                            d_mat_ft=d_mat_ft,
                            mean = 1,
                            std = 2.5,
                            track = True)

list_of_values_w_1 = []
for point in list_of_points_w_1:
    list_of_values_w_1.append(func_value_ft(point) - func_value_ft(x_star_ft))

gamma = 10000*n_ft

list_of_points_w_2 = ProxLora(W_0=W_0_pret, 
                            alpha=1,
                            inner_step_size=0.035/(L_ft+(1./gamma)),
                            iter_max_sub=6,
                            max_iter=500,
                            gamma = gamma,
                            rank=1,
                            d_ft=d_ft,
                            d_mat_ft=d_mat_ft,
                            mean = 1,
                            std = 2.5,
                            track=True)

list_of_values_w_2 = []
for point in list_of_points_w_2:
    list_of_values_w_2.append(func_value_ft(point) - func_value_ft(x_star_ft))



gamma = 1000000*n_ft

list_of_points_w_3 = ProxLora(W_0=W_0_pret, 
                            alpha=1,
                            inner_step_size=0.04/(L_ft+(1./gamma)),
                            iter_max_sub=5,
                            max_iter=600,
                            gamma = gamma,
                            rank=1,
                            d_ft=d_ft,
                            d_mat_ft=d_mat_ft, 
                            mean = 1,
                            std = 2.5,
                            track=True)

list_of_values_w_3 = []
for point in list_of_points_w_3:
    list_of_values_w_3.append(func_value_ft(point) - func_value_ft(x_star_ft))


# list_of_points_w_k_30, list_of_vals_k_30 = RandChain_Lora_Lin(W_0_pret, 
#                                 alpha=1,
#                                 step_size=1/L_ft,
#                                 max_iter=60000,
#                                 rank=30,
#                                 d=d_ft,
#                                 d_mat=d_mat_ft,
#                                 mean = 1,
#                                 std = 2.5,
#                                 )

# list_of_points_w_k_1, list_of_vals_k_1 = RandChain_Lora_Lin(W_0_pret, 
#                                 alpha=1,
#                                 step_size=1/L_ft,
#                                 max_iter=6000,
#                                 rank=2,
#                                 d=d_ft,
#                                 d_mat=d_mat_ft,
#                                 mean = 1,
#                                 std = 2.5,
#                                 )

list_of_points_w_k_10, list_of_vals_k_10 = RandChain_Lora_Lin(W_0_pret, 
                                alpha=1,
                                step_size=1/L_ft,
                                max_iter=3000,
                                rank=1,
                                d=d_ft,
                                d_mat=d_mat_ft,
                                mean = 1,
                                std = 2.5,
                                )
list_of_points_w_k_10_0, list_of_vals_k_10_0 = RandChain_Lora_Lin(W_0_pret, 
                                alpha=1,
                                step_size=3/L_ft,
                                max_iter=3000,
                                rank=1,
                                d=d_ft,
                                d_mat=d_mat_ft,
                                mean = 1,
                                std = 2.5,
                                )

# list_of_points_w_k_20, list_of_vals_k_20 = RandChain_Lora_Lin(W_0_pret, 
#                                 alpha=1,
#                                 step_size=1/L_ft,
#                                 max_iter=60000,
#                                 rank=20,
#                                 d=d_ft,
#                                 d_mat=d_mat_ft,
#                                 mean = 1,
#                                 std = 2.5,
#                                 )

# list_of_points_w_k_1_25, list_of_vals_k_1_25 = RandChain_Lora_Lin(W_0_pret, 
#                                 alpha=1,
#                                 step_size=1/L_ft,
#                                 max_iter=3000,
#                                 rank=1,
#                                 d=d_ft,
#                                 d_mat=d_mat_ft,
#                                 mean = 1,
#                                 std = 25,
#                                 )

# list_of_points_w_k_20_25_10, list_of_vals_k_20_25_10 = RandChain_Lora_Lin(W_0_pret, 
#                                 alpha=1,
#                                 step_size=1/L_ft,
#                                 max_iter=6000,
#                                 rank=2,
#                                 d=d_ft,
#                                 d_mat=d_mat_ft,
#                                 mean = 100,
#                                 std = 250,
#                                 )

# list_of_points_w_k_20_gauss, list_of_vals_k_20_gauss = RandChain_Lora_Lin_Unifrom(W_0_pret, 
#                                 alpha=1,
#                                 step_size=1/L_ft,
#                                 max_iter=6000,
#                                 rank=2,
#                                 d=d_ft,
#                                 d_mat=d_mat_ft
#                                 )

list_of_points_w_k_20_Orth, list_of_vals_k_20_Orth = RandChain_Lora_Lin_Orth(W_0_pret, 
                                alpha=1,
                                step_size=1/L_ft,
                                max_iter=3000,
                                rank=1,
                                d=d_ft,
                                d_mat=d_mat_ft
                                )


# list_of_points_w_prox_20, list_of_vals_w_prox_20  = ProxLora(W_0=W_0_pret, 
#                             alpha=1,
#                             inner_step_size=0.01/(L_ft+(1./gamma)),
#                             iter_max_sub=10000,
#                             max_iter=300,
#                             k_max=1,
#                             gamma = gamma,
#                             rank=1,
#                             d_ft=d_ft,
#                             d_mat_ft=d_mat_ft)

# list_of_norms_w = []
# for point in list_of_points_w:
#     list_of_norms_w.append(np.linalg.norm(point - x_star_ft)**2)

# list_of_points_w_1 = ProxLora(W_0=W_0_pret, 
#                             alpha=1,
#                             inner_step_size=0.01/(L_ft+(1./gamma)),
#                             iter_max_sub=10000,
#                             max_iter=30,
#                             k_max=10,
#                             gamma = gamma,
#                             rank=1,
#                             d_ft=d_ft,
#                             d_mat_ft=d_mat_ft)

# list_of_points_w_2 = ProxLora(W_0=W_0_pret, 
#                             alpha=1,
#                             inner_step_size=0.01/(L_ft+(1./gamma)),
#                             iter_max_sub=10000,
#                             max_iter=15,
#                             k_max=20,
#                             gamma = gamma,
#                             rank=1,
#                             d_ft=d_ft,
#                             d_mat_ft=d_mat_ft)

# list_of_points_w_3 = ProxLora(W_0=W_0_pret, 
#                             alpha=1,
#                             inner_step_size=0.01/(L_ft+(1./n_ft)),
#                             iter_max_sub=10000,
#                             max_iter=30,
#                             k_max=10,
#                             gamma = n_ft,
#                             rank=10,
#                             d_ft=d_ft,
#                             d_mat_ft=d_mat_ft)

# list_of_norms_w_1 = []
# for point in list_of_points_w_1:
#     list_of_norms_w_1.append(np.linalg.norm(point - x_star_ft)**2)

# list_of_values_w_1 = []
# for point in list_of_points_w_1:
#     list_of_values_w_1.append(func_value_ft(point) - func_value_ft(x_star_ft))

# list_of_values_w_2 = []
# for point in list_of_points_w_2:
#     list_of_values_w_2.append(func_value_ft(point) - func_value_ft(x_star_ft))

# list_of_values_w_k_3 = []
# for point in list_of_vals_k_3:
#     list_of_values_w_k_3.append(func_value_ft(point) - func_value_ft(x_star_ft))

# list_of_values_w = []
# for point in list_of_points_w:
#     list_of_values_w.append(func_value_ft(point) - func_value_ft(x_star_ft))



# print(A_finetuned.shape)



print(d_ft)
print(d_mat_ft)

def gd_ft(x_0, gamma, max_iter = 10000):
    x_k = np.reshape(x_0, (d_mat_ft,d_mat_ft))
    list_of_norms = [np.linalg.norm(np.reshape(x_k, (d_ft,)) - x_star_ft) ** 2]
    list_of_points = [x_0]
    list_of_losses = [func_value_ft(x_0) - func_value_ft(x_star_ft)]
    for k in tqdm(range(int(max_iter))):
        x_k -= gamma * np.reshape(grad_full_ft(np.reshape(x_k, (d_ft,))), (d_mat_ft,d_mat_ft)) 
        list_of_norms.append(np.linalg.norm(np.reshape(x_k, (d_ft,)) - x_star_ft) ** 2 )
        list_of_points.append(x_k)
        list_of_losses.append(func_value_ft(np.reshape(x_k, (d_ft,))) - func_value_ft(x_star_ft))

    return list_of_points, list_of_norms, list_of_losses

list_of_points_ft, list_of_norms_ft, list_of_losses_ft = gd_ft(x_star_pret, 1/L_ft, max_iter=3000)
# plt.plot(list_of_norms_ft)
# plt.yscale('log')
# plt.savefig('gd_ft_1.pdf')



# print(list_of_norms_w)
# plt.plot(list_of_values_w, label = 'k_max = 1')
# plt.plot(list_of_values_w_1, label = 'k_max = 10')
plt.plot(list_of_losses_ft, label = 'GD')
# plt.plot(list_of_vals_k_1 - func_value_ft(x_star_ft), label = 'rank=1')
# plt.plot(list_of_vals_k_1_25 - func_value_ft(x_star_ft), label = 'rank=1, std=25')
# plt.plot(list_of_vals_k_20_25_10 - func_value_ft(x_star_ft), label = 'rank=20, std=250, mean = 100')
# plt.plot(list_of_vals_k_20_gauss - func_value_ft(x_star_ft), label = 'rank=20, uni')
plt.plot(list_of_vals_k_10 - func_value_ft(x_star_ft), label = 'rank=1, std = 2.5')
plt.plot(list_of_vals_k_10_0 - func_value_ft(x_star_ft), label = 'rank=1, std = 2.5, tuned')
plt.plot(list_of_vals_k_20_Orth - func_value_ft(x_star_ft), label = 'rank=1, Orth')
plt.plot(list_of_values_w_1, label = 'rank=1, prox, 10000, 3 iter')
plt.plot(list_of_values_w_0, label = 'rank=1, prox, 10000, 1 iter')
plt.plot(list_of_values_w_2, label = 'rank=1, prox, 10000, 6 iter')
plt.plot(list_of_values_w_3, label = 'rank=1, prox, 10000, 5 iter')

# plt.plot(list_of_vals_k_10 - func_value_ft(x_star_ft), label = 'rank=10')
plt.yscale('log')
plt.grid()
# plt.tight_layout()
plt.legend(loc = 'best')
plt.xlabel('# of oracle calls')
plt.ylabel('$f(x^k) - f^*$')
plt.savefig('RandLoRA-Lin_100-gauss-prox.pdf')
























































import numpy as np
import matplotlib.pyplot as plt
from sklearn import datasets
import matplotlib
from tqdm import tqdm
import torch
import copy




n = 2000
d=100

data_matrix, labels = datasets.make_classification(n_samples=n, n_features=d)
labels = 2*labels - 1
regularizer = 0.1
reg  = 0.1

# def individual_log_loss(weights, features, label, regularizer):
#     return np.log(1+np.exp(-label * features @ weights)) + regularizer * np.linalg.norm(weights, 2)**2 / 2

# def individual_log_loss_grad(weights, features, label, regularizer):
#     scaler = - 1. / (1. + np.exp(label * features @ weights))

    # return scaler * label * features + regularizer*weights

def log_loss(weights):

    log_loss_vector = np.log(1. + np.exp(-labels[:, None] * (data_matrix@weights)))
    log_loss = log_loss_vector.mean()

    return log_loss + regularizer*np.linalg.norm(weights, 2)**2/2

def log_loss_grad(weights):

    label_by_features = labels[:, None] * data_matrix
    scalers = - 1. / (1 + np.exp(label_by_features @ weights))

    first_part = (scalers[:,None]*label_by_features).mean(axis = 0)
    second_part = regularizer * weights

    return first_part + second_part

def gradient_descent(start_iterate, stepsize, num_iterations):

    x_cur = np.copy(start_iterate)

    loss_values = [log_loss(x_cur)]
    grad_norm_values = [np.linalg.norm(log_loss_grad(x_cur), 2)**2]
    list_points = [x_cur]

    for i in tqdm(range(num_iterations)):

        grad_ = log_loss_grad(x_cur)
        x_new = x_cur - stepsize * grad_
        loss_values.append(log_loss(x_new))
        grad_norm_values.append(np.linalg.norm(grad_,2)**2)
        list_points.append(x_new)
        x_cur = np.copy(x_new)

    return x_cur, loss_values, grad_norm_values, list_points


def ProxLora(W_0, alpha, inner_step_size, iter_max_sub, max_iter, k_max, gamma, rank, d, d_mat, mean, std):
    current_matrix = W_0
    d_mat = current_matrix.shape[0]
    list_of_points_w = []
    list_of_values_w = []
    
    for t in tqdm(range(max_iter)):
        W_k = copy.deepcopy(current_matrix)
        for k in range(0, k_max):
            # print(k)
            list_of_points_w.append(np.reshape(current_matrix, (d,)))
            list_of_values_w.append(log_loss(np.reshape(current_matrix, (d,))))
            S_k = np.random.normal(mean, std, size=(d_mat, rank))
            current_Z = solve_subproblem(W_k, current_matrix, S_k, iter_max_sub, inner_step_size, gamma, rank, d, d_mat)
            W_k += S_k@current_Z
        current_matrix = current_matrix + alpha*(W_k - current_matrix)
        # list_of_points_w.append(np.reshape(current_matrix, (8,)))
        

    

    return list_of_points_w, list_of_values_w

















def get_constants():
    
    individual_smoothness_constants = []
    for i in range(data_matrix.shape[0]):
        individual_smoothness_constant = 0.25 * np.linalg.norm(data_matrix[i], 2) ** 2 + regularizer
        individual_smoothness_constants.append(individual_smoothness_constant)

    n, d = data_matrix.shape

    objective_function_smoothness_constant = np.linalg.norm(data_matrix.transpose() @ data_matrix / (4*n) + regularizer * np.eye(d), 2 )

    return np.array(individual_smoothness_constants), objective_function_smoothness_constant


def solve_subproblem(W_cur, W, S, iter_max_sub, step_size, gamma, rank, d, d_mat):
    Z_0 = np.zeros((rank, d_mat))
    
    Z_cur = Z_0
    for j in range(iter_max_sub):
        delta = np.reshape(W_cur + S@Z_cur, (d,))
        Z_cur = Z_cur - step_size* S.T @ (np.reshape(log_loss_grad(delta), (d_mat, d_mat)) + (1./gamma)*(W_cur+S@Z_cur - W))
    return Z_cur

def RandChain_Lora(W_0, alpha, step_size, max_iter, rank, d, d_mat, mean, std):
    current_matrix = W_0
    d_mat = current_matrix.shape[0]
    list_of_points_w = []
    list_of_values_w = []
    
    for t in tqdm(range(max_iter)):
        W_k = copy.deepcopy(current_matrix)
        S_k = np.random.normal(mean, std, size=(d_mat, rank))
        delta = np.reshape(W_k, (d,))
        W_k += -step_size * S_k @ np.linalg.inv(S_k.T @ S_k) @ S_k.T @ np.reshape(log_loss_grad(delta), (d_mat, d_mat))
        # for k in range(0, k_max):
        #     # print(k)
        #     list_of_points_w.append(np.reshape(current_matrix, (d,)))
        #     list_of_values_w.append(log_loss(np.reshape(current_matrix, (d,))))
        #     S_k = np.random.normal(mean, std, size=(d_mat, rank))
        #     current_Z = solve_subproblem(W_k, current_matrix, S_k, iter_max_sub, inner_step_size, gamma, rank, d, d_mat)
        #     W_k += S_k@current_Z
        current_matrix = current_matrix + alpha*(W_k - current_matrix)
        list_of_points_w.append(np.reshape(current_matrix, (d,)))
        list_of_values_w.append(log_loss(np.reshape(current_matrix, (d,))))
        # list_of_points_w.append(np.reshape(current_matrix, (8,)))
        

    

    return list_of_points_w, list_of_values_w

reg = 0.1
_, L = get_constants()
x_0 = np.ones(d)


# _, L = get_constants(data_matrix, reg)

d_mat = 10

W_0 = np.reshape(x_0, (d_mat, d_mat))

print(L)
print(reg)

gamma = n/600

list_list_of_points_w_i_k_3 = []
list_list_of_vals_i_k_3 = []

for i in range(1):
    np.random.seed(i)

    list_of_points_w_i_k_3, list_of_vals_i_k_3 = RandChain_Lora(W_0=W_0, 
                                alpha=1,
                                step_size=1/L,
                                max_iter=6000,
                                rank=3,
                                d=d,
                                d_mat=d_mat,
                                mean = 1,
                                std = 2.5,
                                )
    # list_list_of_points_w_i.append(list_of_points_w_i)
    list_list_of_vals_i_k_3.append(list_of_vals_i_k_3)

avg_list_of_vals_1_k_3 = np.mean(list_list_of_vals_i_k_3, axis = 0)

list_list_of_points_w_i_k_1 = []
list_list_of_vals_i_k_1 = []

for i in range(1):
    np.random.seed(i)

    list_of_points_w_i_k_1, list_of_vals_i_k_1 = RandChain_Lora(W_0=W_0, 
                                alpha=1,
                                step_size=1/L,
                                max_iter=6000,
                                rank=1,
                                d=d,
                                d_mat=d_mat,
                                mean = 1,
                                std = 2.5,
                                )
    # list_list_of_points_w_i.append(list_of_points_w_i)
    list_list_of_vals_i_k_1.append(list_of_vals_i_k_1)

avg_list_of_vals_1_k_1 = np.mean(list_list_of_vals_i_k_1, axis = 0)



# list_of_points_w_5, list_of_vals_5 = ProxLora(W_0=W_0, 
#                             alpha=1,
#                             inner_step_size=0.01/(L+(1./gamma)),
#                             iter_max_sub=10000,
#                             max_iter=2,
#                             k_max=5,
#                             gamma = gamma,
#                             rank=1,
#                             d=d,
#                             d_mat=d_mat,
#                             mean = 1,
#                             std = 2.5,
#                             )


# list_of_points_w_10, list_of_vals_10 = ProxLora(W_0=W_0, 
#                             alpha=1,
#                             inner_step_size=0.01/(L+(1./gamma)),
#                             iter_max_sub=10000,
#                             max_iter=1,
#                             k_max=10,
#                             gamma = gamma,
#                             rank=1,
#                             d=d,
#                             d_mat=d_mat,
#                             mean = 1,
#                             std = 2.5,
#                             )

x_star_ft_0, loss_values_gd_ft_0, grad_norm_values_gd_ft_0, list_points_ft_0 = gradient_descent(x_0, 1/L, 6000)

# list_of_values_w_1 = []
# for point in list_of_points_w_1:
#     list_of_values_w_1.append(log_loss(point,data_matrix_ft,labels_ft,reg))


# x_0 = np.ones(d)
# reg = 0.01
# _, L = get_constants(data_matrix, reg)



# print(avg_list_of_vals_1[0:1000] -loss_values_gd_ft_0[-1])
# array = avg_list_of_vals_1[0:1000] -loss_values_gd_ft_0[-1]
# array.tofile('losses.csv', sep = ',')



plt.plot(np.abs(avg_list_of_vals_1_k_1 -loss_values_gd_ft_0[-1]), label = 'k=3')
plt.plot(np.abs(avg_list_of_vals_1_k_3 -loss_values_gd_ft_0[-1]), label = 'k=3, ex')
# plt.plot(list_of_vals_10 -loss_values_gd_ft_0[-1], label = 'k=10')
plt.plot(loss_values_gd_ft_0 -loss_values_gd_ft_0[-1], label = 'GD-full')
# plt.plot(loss_values_gd_ft_0[:-1700] - loss_values_gd_ft_0[-1])
plt.legend(loc = 'best')

plt.yscale('log')
plt.grid()
plt.savefig('new_test_avg_1.pdf')


# print(log_loss(list_points[0], data_matrix, labels, reg) - log_loss(list_points[-1], data_matrix, labels, reg))


# plt.plot(list_of_vals)
# plt.yscale('log')
# plt.grid()
# plt.savefig('test_log_reg_gd_4.pdf')

# print(log_loss(np.ones(d), data_matrix_ft, labels_ft, reg))




==> tables/results-roberta-base-rank=4.tex <==
\begin{table*}[htb!]
\resizebox{\textwidth}{!}{%
\centering
{
\begin{tabular}{lcc|ccccc|c}
 \thickhline
\multirow{2}{*}{Method} & \multirow{2}{*}{\# Iterations} & \multirow{2}{*}{\# Epochs} & \multicolumn{6}{c}{GLUE}  \\ 
 & & & \textcolor{black}{SST-2} &
 \textcolor{black}{MRPC} & \textcolor{black}{CoLA} &
 \textcolor{black}{RTE} & \textcolor{black}{STS-B} & 
 Avg.\\
 \hline
LoRA & 1 & 20 
& 
&
&
&
73.3\textsubscript{$\pm$0.8} & 
& 
\\
 
ALoRA & 1 & 20
& 
&
&
&
71.0\textsubscript{$\pm$0.5} & 
& 
\\

\cdashline{1-9}
\multirow{2}{*}{COLA} & 2 & 10
& 
&
&
&
& 
& 
\\
& 10 & 2 
& 
&
&
&
& 
& 
\\

\cdashline{1-9}
\multirow{2}{*}{RAC-LoRA} & 2 & 10
& 
&
&
&
& 
& 
\\
& 10 & 2
& 
&
&
&
& 
& 
\\

\\[-2.5ex]
\hline
LoRA & 1 & 50 
& 
&
&
&
73.9\textsubscript{$\pm$1.9} & 
& 
\\
 
ALoRA & 1 & 50
& 
&
&
&
71.7\textsubscript{$\pm$1.2} & 
& 
\\

\cdashline{1-9}
\multirow{2}{*}{COLA} & 5 & 10
& 
&
&
&
& 
& 
\\
& 10 & 5 
& 
&
&
&
& 
& 
\\

\cdashline{1-9}
\multirow{2}{*}{RAC-LoRA} & 5 & 10
& 
&
&
&
& 
& 
\\
& 10 & 5
& 
&
&
&
& 
& 
\\

\hline
LoRA & 1 & 100 
& 
&
&
&
73.9\textsubscript{$\pm$1.7} & 
& 
\\
 
ALoRA & 1 & 100
& 
&
&
&
74.2\textsubscript{$\pm$1.1} & 
& 
\\

COLA & 10 & 10
& 
&
&
&
& 
& 
\\

RAC-LoRA & 10 & 10
& 
&
&
&
& 
& 
\\


\thickhline
\end{tabular}
}
}

\caption{\textbf{Performance of the methods using RoBERTa-base for rank 4}. The experiments are based on 5 GLUE datasets. We report Matthews correlation coefficient for CoLA, Pearson correlation coefficient for STS-B, and accuracy for the remaining tasks, with the standard deviations given in the subscript. The best performance per rank is highlighted by bold.}\label{results_roberta_base_rank=4}
\vspace{-5.0pt}
\end{table*}

==> tables/results-roberta-base-rank=8.tex <==
\begin{table*}[htb!]
\resizebox{\textwidth}{!}{%
\centering
{
\begin{tabular}{lcc|ccccc|c}
 \thickhline
\multirow{2}{*}{Method} & \multirow{2}{*}{\# Iterations} & \multirow{2}{*}{\# Epochs} & \multicolumn{6}{c}{GLUE}  \\ 
 & & & \textcolor{black}{SST-2} &
 \textcolor{black}{MRPC} & \textcolor{black}{CoLA} &
 \textcolor{black}{RTE} & \textcolor{black}{STS-B} & 
 Avg.\\
 \hline
LoRA & 1 & 20 
& 
&
&
&
73.5\textsubscript{$\pm$0.9} & 
& 
\\
 
ALoRA & 1 & 20
& 
&
&
&
71.4\textsubscript{$\pm$0.3} & 
& 
\\

\cdashline{1-9}
\multirow{2}{*}{COLA} & 2 & 10
& 
&
&
&
& 
& 
\\
& 10 & 2 
& 
&
&
&
& 
& 
\\

\cdashline{1-9}
\multirow{2}{*}{RAC-LoRA} & 2 & 10
& 
&
&
&
& 
& 
\\
& 10 & 2
& 
&
&
&
& 
& 
\\

\\[-2.5ex]
\hline
LoRA & 1 & 50 
& 
&
&
&
74.2\textsubscript{$\pm$1.9} & 
& 
\\
 
ALoRA & 1 & 50
& 
&
&
&
73.6\textsubscript{$\pm$2.3} & 
& 
\\

\cdashline{1-9}
\multirow{2}{*}{COLA} & 5 & 10
& 
&
&
&
& 
& 
\\
& 10 & 5 
& 
&
&
&
& 
& 
\\

\cdashline{1-9}
\multirow{2}{*}{RAC-LoRA} & 5 & 10
& 
&
&
&
& 
& 
\\
& 10 & 5
& 
&
&
&
& 
& 
\\

\hline
LoRA & 1 & 100 
& 
&
&
&
75.5\textsubscript{$\pm$0.8} & 
& 
\\
 
ALoRA & 1 & 100
& 
&
&
&
73.3\textsubscript{$\pm$2.7} & 
& 
\\

COLA & 10 & 10
& 
&
&
&
& 
& 
\\

RAC-LoRA & 10 & 10
& 
&
&
&
& 
& 
\\


\thickhline
\end{tabular}
}
}

\caption{\textbf{Performance of the methods using RoBERTa-base for rank 8}. The experiments are based on 5 GLUE datasets. We report Matthews correlation coefficient for CoLA, Pearson correlation coefficient for STS-B, and accuracy for the remaining tasks, with the standard deviations given in the subscript. The best performance per rank is highlighted by bold.}\label{results_roberta_base_rank=8}
\vspace{-5.0pt}
\end{table*}

==> tables/results-roberta-large-rank=2.tex <==
\begin{table*}[htb!]
\resizebox{\textwidth}{!}{%
\centering
{
\begin{tabular}{lcc|ccccc|c}
 \thickhline
\multirow{2}{*}{Method} & \multirow{2}{*}{\# Iterations} & \multirow{2}{*}{\# Epochs} & \multicolumn{6}{c}{GLUE}  \\ 
 & & & \textcolor{black}{SST-2} &
 \textcolor{black}{MRPC} & \textcolor{black}{CoLA} &
 \textcolor{black}{RTE} & \textcolor{black}{STS-B} & 
 Avg.\\
 \hline
LoRA & 1 & 20 
& 
&
&
&
82.4\textsubscript{$\pm$0.6} & 
& 
\\
 
ALoRA & 1 & 20
& 
&
&
&
78.6\textsubscript{$\pm$0.5} & 
& 
\\

\cdashline{1-9}
\multirow{2}{*}{COLA} & 2 & 10
& 
&
&
&
& 
& 
\\
& 10 & 2 
& 
&
&
&
& 
& 
\\

\cdashline{1-9}
\multirow{2}{*}{RAC-LoRA} & 2 & 10
& 
&
&
&
& 
& 
\\
& 10 & 2
& 
&
&
&
& 
& 
\\

\\[-2.5ex]
\hline
LoRA & 1 & 50 
& 
&
&
&
83.0\textsubscript{$\pm$0.8} & 
& 
\\
 
ALoRA & 1 & 50
& 
&
&
&
83.4\textsubscript{$\pm$0.8} & 
& 
\\

\cdashline{1-9}
\multirow{2}{*}{COLA} & 5 & 10
& 
&
&
&
& 
& 
\\
& 10 & 5 
& 
&
&
&
& 
& 
\\

\cdashline{1-9}
\multirow{2}{*}{RAC-LoRA} & 5 & 10
& 
&
&
&
& 
& 
\\
& 10 & 5
& 
&
&
&
& 
& 
\\

\hline
LoRA & 1 & 100 
& 
&
&
&
84.1\textsubscript{$\pm$2.2} & 
& 
\\
 
ALoRA & 1 & 100
& 
&
&
&
85.0\textsubscript{$\pm$1.2} & 
& 
\\

COLA & 10 & 10
& 
&
&
&
& 
& 
\\

RAC-LoRA & 10 & 10
& 
&
&
&
& 
& 
\\


\thickhline
\end{tabular}
}
}

\caption{\textbf{Performance of the methods using RoBERTa-large for rank 2}. The experiments are based on 5 GLUE datasets. We report Matthews correlation coefficient for CoLA, Pearson correlation coefficient for STS-B, and accuracy for the remaining tasks, with the standard deviations given in the subscript. The best performance per rank is highlighted by bold.}\label{results_roberta_large_rank=2}
\vspace{-5.0pt}
\end{table*}

==> tables/results-roberta-large-rank=4.tex <==
\begin{table*}[htb!]
\resizebox{\textwidth}{!}{%
\centering
{
\begin{tabular}{lcc|ccccc|c}
 \thickhline
\multirow{2}{*}{Method} & \multirow{2}{*}{\# Iterations} & \multirow{2}{*}{\# Epochs} & \multicolumn{6}{c}{GLUE}  \\ 
 & & & \textcolor{black}{SST-2} &
 \textcolor{black}{MRPC} & \textcolor{black}{CoLA} &
 \textcolor{black}{RTE} & \textcolor{black}{STS-B} & 
 Avg.\\
 \hline
LoRA & 1 & 20 
& 
&
&
&
84.2\textsubscript{$\pm$1.0} & 
& 
\\
 
ALoRA & 1 & 20
& 
&
&
&
81.6\textsubscript{$\pm$1.8} & 
& 
\\

\cdashline{1-9}
\multirow{2}{*}{COLA} & 2 & 10
& 
&
&
&
&
& 
\\
& 10 & 2 
& 
&
&
&
&
& 
\\

\cdashline{1-9}
\multirow{2}{*}{RAC-LoRA} & 2 & 10
& 
&
&
&
&
& 
\\
& 10 & 2
& 
&
&
&
&
& 
\\

\\[-2.5ex]
\hline
LoRA & 1 & 50 
& 
&
&
&
72.1\textsubscript{$\pm$17.5} & 
& 
\\
 
ALoRA & 1 & 50
& 
&
&
&
83.5\textsubscript{$\pm$0.5} & 
& 
\\

\cdashline{1-9}
\multirow{2}{*}{COLA} & 5 & 10
& 
&
&
&
&
& 
\\
& 10 & 5 
& 
&
&
&
&
& 
\\

\cdashline{1-9}
\multirow{2}{*}{RAC-LoRA} & 5 & 10
& 
&
&
&
&
& 
\\
& 10 & 5
& 
&
&
&
&
& 
\\

\hline
LoRA & 1 & 100 
& 
&
&
&
85.0\textsubscript{$\pm$0.5} & 
& 
\\
 
ALoRA & 1 & 100
& 
&
&
&
85.0\textsubscript{$\pm$0.2} & 
& 
\\

COLA & 10 & 10
& 
&
&
&
&
& 
\\

RAC-LoRA & 10 & 10
& 
&
&
&
&
& 
\\


\thickhline
\end{tabular}
}
}

\caption{\textbf{Performance of the methods using RoBERTa-large for rank 4}. The experiments are based on 5 GLUE datasets. We report Matthews correlation coefficient for CoLA, Pearson correlation coefficient for STS-B, and accuracy for the remaining tasks, with the standard deviations given in the subscript. The best performance per rank is highlighted by bold.}\label{results_roberta_large_rank=4}
\vspace{-5.0pt}
\end{table*}

==> tables/results-roberta-large-rank=8.tex <==
\begin{table*}[htb!]
\resizebox{\textwidth}{!}{%
\centering
{
\begin{tabular}{lcc|ccccc|c}
 \thickhline
\multirow{2}{*}{Method} & \multirow{2}{*}{\# Iterations} & \multirow{2}{*}{\# Epochs} & \multicolumn{6}{c}{GLUE}  \\ 
 & & & \textcolor{black}{SST-2} &
 \textcolor{black}{MRPC} & \textcolor{black}{CoLA} &
 \textcolor{black}{RTE} & \textcolor{black}{STS-B} & 
 Avg.\\
 \hline
LoRA & 1 & 20 
& 
&
&
&
83.8\textsubscript{$\pm$0.5} & 
& 
\\
 
ALoRA & 1 & 20
& 
&
&
&
83.3\textsubscript{$\pm$1.6} & 
& 
\\

\cdashline{1-9}
\multirow{2}{*}{COLA} & 2 & 10
& 
&
&
&
&
& 
\\
& 10 & 2 
& 
&
&
&
&
& 
\\

\cdashline{1-9}
\multirow{2}{*}{RAC-LoRA} & 2 & 10
& 
&
&
&
&
& 
\\
& 10 & 2
& 
&
&
&
&
& 
\\

\\[-2.5ex]
\hline
LoRA & 1 & 50 
& 
&
&
&
83.4\textsubscript{$\pm$0.3} & 
& 
\\
 
ALoRA & 1 & 50
& 
&
&
&
84.7\textsubscript{$\pm$1.8} & 
& 
\\

\cdashline{1-9}
\multirow{2}{*}{COLA} & 5 & 10
& 
&
&
&
&
& 
\\
& 10 & 5 
& 
&
&
&
&
& 
\\

\cdashline{1-9}
\multirow{2}{*}{RAC-LoRA} & 5 & 10
& 
&
&
&
&
& 
\\
& 10 & 5
& 
&
&
&
&
& 
\\

\hline
LoRA & 1 & 100 
& 
&
&
&
85.6\textsubscript{$\pm$0.8} & 
& 
\\
 
ALoRA & 1 & 100
& 
&
&
&
83.4\textsubscript{$\pm$1.3} & 
& 
\\

COLA & 10 & 10
& 
&
&
&
&
& 
\\

RAC-LoRA & 10 & 10
& 
&
&
&
&
& 
\\


\thickhline
\end{tabular}
}
}

\caption{\textbf{Performance of the methods using RoBERTa-large for rank 8}. The experiments are based on 5 GLUE datasets. We report Matthews correlation coefficient for CoLA, Pearson correlation coefficient for STS-B, and accuracy for the remaining tasks, with the standard deviations given in the subscript. The best performance per rank is highlighted by bold.}\label{results_roberta_large_rank=8}
\vspace{-5.0pt}
\end{table*}


